Better Sparsifiers for Directed Eulerian Graphs

Spectral sparsification for directed Eulerian graphs is a key component in the design of fast algorithms for solving directed Laplacian linear systems. Directed Laplacian linear system solvers are crucial algorithmic primitives to fast computation of fundamental problems on random walks, such as computing stationary distribution, hitting and commute time, and personalized PageRank vectors. While spectral sparsification is well understood for undirected graphs and it is known that for every graph $G,$ $(1+\varepsilon)$-sparsifiers with $O(n\varepsilon^{-2})$ edges exist [Batson-Spielman-Srivastava, STOC '09] (which is optimal), the best known constructions of Eulerian sparsifiers require $\Omega(n\varepsilon^{-2}\log^4 n)$ edges and are based on short-cycle decompositions [Chu et al., FOCS '18]. In this paper, we give improved constructions of Eulerian sparsifiers, specifically: 1. We show that for every directed Eulerian graph $\vec{G},$ there exist an Eulerian sparsifier with $O(n\varepsilon^{-2} \log^2 n \log^2\log n + n\varepsilon^{-4/3}\log^{8/3} n)$ edges. This result is based on combining short-cycle decompositions [Chu-Gao-Peng-Sachdeva-Sawlani-Wang, FOCS '18, SICOMP] and [Parter-Yogev, ICALP '19], with recent progress on the matrix Spencer conjecture [Bansal-Meka-Jiang, STOC '23]. 2. We give an improved analysis of the constructions based on short-cycle decompositions, giving an $m^{1+\delta}$-time algorithm for any constant $\delta > 0$ for constructing Eulerian sparsifiers with $O(n\varepsilon^{-2}\log^3 n)$ edges.

==> abstract.tex <==
\begin{abstract}
  Spectral sparsification for directed Eulerian graphs is a key
  component in the design of fast algorithms for solving directed
  Laplacian linear systems.
  Directed Laplacian linear system solvers are crucial algorithmic primitives to
  fast computation of fundamental problems on random walks, such as
  computing stationary distribution, hitting and commute time, and personalized
  PageRank vectors.
  While spectral sparsification is well understood for undirected
  graphs and it is known that for every graph $G,$
  $(1+\varepsilon)$-sparsifiers with $O(n\varepsilon^{-2})$ edges
  exist [Batson-Spielman-Srivastava, STOC '09] (which is optimal), the
  best known constructions of Eulerian sparsifiers require
  $\Omega(n\varepsilon^{-2}\log^4 n)$ edges and are based on
  short-cycle decompositions [Chu et al., FOCS '18].

  In this paper, we give improved constructions of Eulerian
  sparsifiers, specifically:
  \begin{enumerate}
    \item We show that for every directed Eulerian graph $\vec{G},$ there exist
      an Eulerian sparsifier with
      $O(n\varepsilon^{-2} \log^2 n \log^2\log n +
      n\varepsilon^{-4/3}\log^{8/3} n)$ edges.  This result is based on
      combining short-cycle decompositions
      [Chu-Gao-Peng-Sachdeva-Sawlani-Wang, FOCS '18, SICOMP] and
      [Parter-Yogev, ICALP'19], with recent progress on the matrix
      Spencer conjecture [Bansal-Meka-Jiang, STOC'23].
    \item We give an improved analysis of the constructions based on
          short-cycle decompositions,
    giving an $m^{1+\delta}$-time
    algorithm for any constant $\delta > 0$ for constructing Eulerian sparsifiers with
    $O(n\varepsilon^{-2}\log^3 n)$ edges.
  \end{enumerate}
\end{abstract}


==> fast.tex <==
\section{Nearly linear time sparsifier}
\label{sec:fast}

\begin{definition}
    Given $\phi, \gamma$ and an undirected graph $G$, a $(\phi,
    \gamma)$-expander decomposition of $G$ is a partition of the vertices $V_1,
    \ldots V_t$ such for all $i$, $\Phi_{G[V_i]} \geq \phi$ and \anvith{Probably need to clarify notation at some point. Just adding some stuff preliminaries} $\sum_i
    w(\partial(V_i)) \leq \gamma \cdot d(V)$.
\end{definition}

\begin{theorem}(\cite{ADK22})
    There is an algorithm \ED that given an unweighted undirected graph $G$
    returns a $(O(\log^2 m), O(1))$-expander
    decomposition of $G$ with high probability in $\ted(m) = O(m\log^7 m)$ time
\end{theorem}

\subsection{Random sampling sparsification}
\label{subsec:sampling}



\Znote{Move the following to preliminaries later}
We let $\DD^{(i)}$ and $\DD^{(o)}$ denote the in and out degree matrices of an directed
graph $\ora{G}$.
They are distinguished only when necessary, otherwise we always refer $\DD$ to
$\DD^{(o)}$.
Then, their corresponding vectors $\dd_o = \AA^\top 1$ and $\dd_i = \AA 1$.
We can write $\LL_{\ora{G}} = \BB^\top \WW \TT$ where $\BB$ is the edge-vertex
transfer matrix and $\TT$ is the incidence matrix for tails of directed edges.
Let the matrix $\HH$ is the incidence matrix for heads of directed edges. 
Then $\BB = \TT - \HH$, $\dd_i = \HH^\top \WW 1$ and $\dd_o = \TT^\top \WW 1$.
For an directed edge $e = (u,v)$ we set $h(e) = v$ be the head of $e$ and $t(e)
= u$ be the tail of $e$.


\begin{algorithm}[t]
    \caption{Random sampling algorithm}
    \label{alg:randomsample}
    \Pro{\SS{$\ora{G},\epsilon$}}{
        \KwIn{An unweighted directed graph $\ora{G}$,
            an error parameter $\epsilon \in (0,1/2)$.
        }
        $\ora{H} \gets \ora{G}$.
        Compute $\rr$ a 1.2-approximate effective resistances in $G$.\;
        \While{$m' \geq O(\epsilon^{-2} n \log n)$}{
            $\ora{H} \gets$ \SSO{$\ora{H},\rr$}\;
        }
        $\ora{H} \gets$ \PD{$\ora{H}, \dd_i, \dd_o$} where $\dd_i$ and $\dd_o$
        are in and out degrees of $\ora{G}$.\;
        \Return{$\ora{H}$.}\;
    }
\end{algorithm}

\begin{algorithm}[t]
    \caption{Random sampling once}
    \label{alg:randomsampleonce}
    \Pro{\SSO{$\ora{G},\rr$}}{
        \KwIn{A directed multi-graph $\ora{G}$ where edge weights are integral
            powers of 2 with largest power $2^q = O(n)$,
            a 2-approximate effective resistances of $G$.
        }
        $\ora{H} \gets \ora{G}$ with only the edges which satisfy $w_e r_e >
        \frac{8n}{m}$ or $\frac{w_e}{(d_i)_{h(e)}} > \frac{4n}{m}$ or
        $\frac{w_e}{(d_o)_{t(e)}} > \frac{4n}{m}$ 
        and remove these edges from $\ora{G}$.\;
        \For{each edge $e \in \ora{G}$}{
            With probability $1/2$, add this edge to $\ora{H}$ with double the
            weight.\;
        }
        \Return{$\ora{H}$.}\;
    }
\end{algorithm}

\begin{algorithm}[t]
    \caption{Degree patching}
    \label{alg:patching}
    \Pro{\PD{$\ora{G}, \dd_i, \dd_o$}}{
        \KwIn{A directed multi-graph $\ora{G}$ where edge weights are integral.
        }
        Write $\ora{G} = \BB^\top \WW \TT$.\;
        Denote $\hat{\dd}_i, \hat{\dd}_o$ be the in and out degrees of
        $\ora{G}$.\;
        Compute a 2-approximate routing $\ff$ for 
        $\min_{\ff} \| \WW^+ \ff \|_\infty$
        subject to $\BB^\top \ff = (\dd_o - \hat{\dd}_o) - (\dd_i -
        \hat{\dd}_i)$.\;
        Find an integral rounding $\ff'$ of $\ff$.\;
        \Return{$\BB^\top \diag{\ff'} \TT$.}\;
    }
\end{algorithm}


For a directed graph $\ora{G}$, its corresponding undirected $G$ has Laplacian
$\frac{1}{2} \BB^\top \WW \BB$.
Note that for Eulerian graph, this definition is that same as
$\frac{1}{2}(\LL_{\ora{G}} + \LL_{\ora{G}}^\top)$.
Let 
$\PPi_u = \frac{1}{2} \WW^{1/2} \BB \LL_G^+ \BB^\top \WW^{1/2}$, 
$\PPi_o = \WW^{1/2} \TT (\DD^{(o)})^+ \TT^\top \WW^{1/2}$ and
$\PPi_i = \WW^{1/2} \HH (\DD^{(i)})^+ \HH^\top \WW^{1/2}$.
Then, $\PPi_u,\PPi_o,\PPi_i$ are all orthogonal projection matrices with
rank $n-1,n,n$ respectively.

\begin{lemma}
    Given directed (non necessarily Eulerian) graph $\ora{G}$ where edge weights
    are integral powers of 2 and a 2-approximate effective resistance $\rr$ in
    $G$, the algorithm \SSO returns a directed graph $\ora{H}$ with edge weights
    still being power of 2 such that if $m = \Omega(n\log n)$, then with high
    probability, the number of edges in $\ora{H}$ is at most $\frac{15}{16}m$
    and
    \begin{align*}
        \| \LL_G^{+/2} (\LL_{\ora{G}} - \LL_{\ora{H}}) (\DD_{\ora{G}}^{(o)})^{+/2} \| \leq 
        O\left( \sqrt{\frac{n\log n}{m}} \right),\\
        \| (\DD_{\ora{G}}^{(o)})^+ (\DD_{\ora{G}}^{(o)} - \DD_{\ora{H}}^{(o)}) \vone \|_\infty \leq 
        O\left( \sqrt{\frac{n\log n}{m}} \right),\\
        \| (\DD_{\ora{G}}^{(i)})^+ (\DD_{\ora{G}}^{(i)} - \DD_{\ora{H}}^{(i)}) \vone \|_\infty \leq 
        O\left( \sqrt{\frac{n\log n}{m}} \right).
    \end{align*}
    The algorithm runs in $O(m)$ time.
\end{lemma}
\begin{proof}
    For simplicity, we denote $\UU = \LL_G, \DD_o = \DD^{(o)}_G$ and $\DD_i =
    \DD^{(i)}_G$.
    Let $r^*_e = \bb_e^\top \UU^+ \bb_e$ be the true effective resistance of an
    edge $e$ in the corresponding undirected graph $G$.

    Since $\rr$ is 2-approximate effective resistances in $G$, each edge $e \in
    G$ satisfies $\lev_G(e) \leq 2 w_e r_w \leq \frac{8n}{m}$ after the
    first step.
    Let $\XX_e$ be the matrix random variable corresponding to edge $e$ such
    that,
    \[
        \XX_e = 
        \begin{cases}
            w_e \UU^{+/2} \bb_e^\top \ee_{t(e)} \DD_o^{+/2}  & \mbox{w.p. } 1/2 \\
            -w_e \UU^{+/2} \bb_e^\top \ee_{t(e)} \DD_o^{+/2}   & \mbox{w.p. } 1/2 \\
        \end{cases}.
    \]
    For any $e$, \anvith{just wondering, what's the bound on $w_e/(d_o)_{h(e)}$ used here? I feel like it's meant to be $(d_o)_{t(e)}$ so the bound is actually $\leq 1$}
    \[
        \| w_e \UU^{+/2} \bb_e^\top \ee_{t(e)} \DD_o^{+/2} \|
        \leq 
        \sqrt{\lev(e)} \cdot \sqrt{w_e/(d_o)_{h(e)}}
        \leq
        O(n/m)
    \]
    Consider the variance term, \anvith{some typos in the transposes in the second formula I think but it's fixed in the next inequality}
    \[
        \sum_e \av \XX_e^* \XX_e 
        =
        \sum_e w_e^2 \cdot \DD_o^{+/2} \ee_{t(e)} \bb_e^\top
        \UU^+ \bb_e^\top \ee_{t(e)} \DD_o^{+/2}
        \leq
        O(n/m) \cdot \sum_e w_e
        \DD_o^{+/2} \ee_{t(e)}^\top \ee_{t(e)} \DD_o^{+/2}
        \preceq
        O(n/m) \II,
    \]
    and \anvith{I think forgot to switch the conjugates in the first formula, but corrected in the second formula}
    \[
        \sum_e \av \XX_e^* \XX_e 
        =
        \sum_e w_e^2 \cdot \UU^{+/2} \bb_e \ee_{t(e)}^\top \DD_o^+
        \ee_{t(e)} \bb_e^\top \UU^{+/2}
        \leq
        O(n/m) \cdot \sum_e w_e 
        \UU^{+/2} \bb_e^\top \bb_e \UU^{+/2}
        \preceq
        O(n/m) \II.
    \]
    We can apply \Cref{thm:bernstein} with $R=O(n/m)$ and $\sigma = O(n/m)$.
    Since $m = \Omega(n\log n)$, with probability $1- n^{-O(1)}$, we get the
    desired error bound.

    We prove the inequality for $\| (\DD_{\ora{G}}^{(i)})^+ \DD_{\ora{H}}^{(i)}
    \vone \|_\infty$.
    The rest follows a similar proof.
    Notice that 
    $\| (\DD_{\ora{G}}^{(i)})^+ \DD_{\ora{H}}^{(i)} \vone \|_\infty = 
    \| (\DD_{\ora{G}}^{(i)})^+ \DD_{\ora{H}}^{(i)} \|$.
    Let $\YY_e$ be the matrix random variable corresponding to edge $e$
    \[
        \YY_e = 
        \begin{cases}
            w_e \DD_i^+ \ee_{t(e)} \ee_{t(e)}^\top & \mbox{w.p. } 1/2 \\
            -w_e \DD_i^+ \ee_{t(e)} \ee_{t(e)}^\top  & \mbox{w.p. } 1/2 \\
        \end{cases}.
    \]
    For any $e$,
    \[
        \| w_e \DD_i^+ \ee_{t(e)} \ee_{t(e)}^\top \|
        =
        \frac{w_e}{(d_o)_{h(e)}}
        \leq
        O(n/m)
    \]
    The variance terms are
    \[
        \sum_e \av \YY_e^* \YY_e 
        =
        \sum_e \av \YY_e \YY_e^*
        =
        \sum_e w_e^2 \cdot \DD_i^+ \ee_{t(e)} \ee_{t(e)}^\top \DD_i^+
        \leq
        O(n/m) \cdot \sum_e w_e 
        \DD_i^+ \ee_{t(e)}^\top \ee_{t(e)} 
        \preceq 
        O(n/m) \II,
    \]
    Then applying \Cref{thm:bernstein} with $R = O(n/m)$ and $\sigma = O(n/m)$
    gives with high probability the desired error bound 
    $\| (\DD_{\ora{G}}^{(i)})^+ \DD_{\ora{H}}^{(i)} \vone \|_\infty \leq 
    O(\sqrt{n\log n/ m})$.

    Consider the number of edges in $\ora{H}$.
    Since
    \begin{align*}
        \sum_e w_e r_e \leq 2 \sum_e w_e r^*_e =
        2 \tr{\PPi_u} &= 2n-2,  \\
        \sum_e w_e / (d_o)_{t(e)} &= n, \\
        \sum_e w_e / (d_i)_{h(e)} &= n,
    \end{align*}
    the number of edges removed initialy is at most $\frac{3}{4}m$. 
    The expected fraction of edges that are added by the random sampling step is
    $\frac{1}{2}$. 
    As long as $m = \Omega(n)$, by a Chernoff bound, at most $\frac{3}{4}$
    fraction of the remaining edges are added to $\ora{H}$, giving us
    at least $\frac{1}{16}m$ removed as required.
\end{proof}






\begin{lemma}[\cite{Coh95}]
    Given a network $\mathcal{N}$ with integral capacities and a fractional flow
    $\ff$, there is an algorithm that finds an integral flow $\ff'$ with no
    worse cost than $\ff$ in time $O(m \log n)$.
\end{lemma}

\begin{lemma}[\cite{She13}]
    For of a graph of conductance $\phi$, the minimum congestion for any demand
    $d$ is at most $\phi^{-1} \| d \|_\infty$.
\end{lemma}

\begin{lemma}[\cite{She13}]
    There is an algorithm that given a graph of conductance $\phi$, computes
    $(1+\epsilon)$-approximate minimum congestion flow in time 
    $O(m\epsilon^{-2} \phi^{-1} \log^2 n)$.
\end{lemma}


==> svapprox.tex <==
\section{Sparsifier for singular value approximation}
\label{sec:svapprox}


\anvith{@me add 3.1,3.5,3.7,3.18 from \cite{ahmadinejad2023singular}}

\begin{definition}[Definition 3.1 in \cite{ahmadinejad2023singular}] Let $\mathbf{A},\tilde{\mathbf{A}} \in \mathbb{C}^{m \times n}$ and $\mathbf{E} \in \mathbb{C}^{m\times m}$, $\mathbf{F} \in \mathbb{C}^{n\times n}$ be PSD matrices. For $\epsilon \geq 0$ we say $\tilde{\mathbf{A}}$ is an $\epsilon$-approximation of $\mathbf{A}$ with respect to error matrices $\mathbf{E}$ and $\mathbf{F}$ if any of the following equivalent conditions hold:

\begin{enumerate}
    \item $| x* (\mathbf{A} - \tilde{\mathbf{A}}) y| \leq \frac{\epsilon}{2} (x* \mathbf{E} X + y* \mathbf{F} y)$ for all $x \in \mathbb{C}^m,y \in \mathbb{C}^n$
\end{enumerate}

\end{definition}
